Sympiler: Transforming Sparse Matrix Codes by Decoupling Symbolic Analysis

Sympiler is a domain-specific code generator that optimizes sparse matrix computations by decoupling the symbolic analysis phase from the numerical manipulation stage in sparse codes. The computation patterns in sparse numerical methods are guided by the input sparsity structure and the sparse algorithm itself. In many real-world simulations, the sparsity pattern changes little or not at all. Sympiler takes advantage of these properties to symbolically analyze sparse codes at compile-time and to apply inspector-guided transformations that enable applying low-level transformations to sparse codes. As a result, the Sympiler-generated code outperforms highly-optimized matrix factorization codes from commonly-used specialized libraries, obtaining average speedups over Eigen and CHOLMOD of 3.8X and 1.5X respectively.

==> Figures/codestyle.tex <==
\lstset{ %
language=C++,                % choose the language of the code
basicstyle=\ttfamily\footnotesize,       % the size of the fonts that are used for the code
columns=fullflexible,
numbers=left,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it is 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
%backgroundcolor=\color{codeBG3},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,           % adds a frame around the code
tabsize=2,          % sets default tabsize to 2 spaces
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=false,    % sets if automatic breaks should only happen at whitespace
escapeinside={\%*}{*)},          % if you want to add a comment within your code
keywordstyle=\color{blue},       % keyword style
  %language=Octave,                 % the language of the code
  otherkeywords={SearchVar,MV,TSS,tileExpr,Search,tFunc...},           % if you want to add more keywords to the set
  numberstyle=\tiny\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},
  escapechar=|
}



==> SRC/artifact.tex <==
\input{artifactCodeStyle}
\appendix
\section{Artifact Description: Sympiler: Transforming Sparse Matrix Codes by Decoupling Symbolic Analysis}


%Submission and reviewing guidelines and methodology: \\
%{\small\em http://sc17.supercomputing.org/submitters/technical-papers/reproducibility-initiatives-for-technical-papers/artifact-description-paper-title/}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

{\em This artifact provides information to reproduce results shown in the paper: ``Sympiler: Transforming Sparse Matrix Codes by Decoupling Symbolic Analysis''. We explain how to compile and run Sympiler and also provide instructions to build the CHOLMOD and Eigen libraries used for comparison. For convenience, a script for evaluating each algorithm in the paper is provided.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{Check-list (artifact meta-information)}

%{\em Fill in whatever is applicable with some informal keywords and remove the rest}

{\small
\begin{itemize}
  \item {\bf Algorithm: The sparse Cholesky factorization and the triangular solver with a sparse right-hand-side}
  \item {\bf Program: C++ code}
  \item {\bf Compilation: GCC v.5.4.0 with -O3 flag.}
  %\item {\bf Transformations: }
  \item {\bf Binary: OpenBLAS v.0.2.19}
  \item {\bf Data set: Publicly available matrix market files }
  \item {\bf Run-time environment: Ubuntu 16.04}
  \item {\bf Hardware: Intel\textregistered Core\texttrademark i7-5820K }
  %\item {\bf Run-time state: }
  %\item {\bf Execution:  }
  \item {\bf Output: The L-factor for the Cholesky algorithm and the solution vector $x$ for the triangular solver.}
  \item {\bf Experiment workflow: Install OpenBlas, CholMod, and Eigen. Compile Sympiler and execute the test scripts.}
  \item {\bf Experiment customization: Some parameters need to be changed in CholMod. }
  \item {\bf Publicly available?: yes, to maintain anonymity it will be released after the review process.
}
\end{itemize}
}

\subsubsection{How software can be obtained (if available)}

Sympiler's code will be available in Github. We will provide a link when accepted. To maintain anonymity is not ready for public release.


\subsubsection{Hardware dependencies}
There is not hardware dependency for Sympiler. It compiles and runs on any x86 processor. However, the reported results are obtained on an Intel\textregistered Core\texttrademark i7-5820K.

\subsubsection{Software dependencies}
The current version of Sympiler relies on BLAS for evaluating dense sub-blocks in Cholesky. %The libraries that are used for comparison which are CholMod and Eigen, can also be installed for 

\subsubsection{Datasets}
The current version of Sympiler only supports input matrices in the \textit{matrix market} format. All matrices selected for evaluation are publicly available from the Florida Sparse Matrix Repository. The matrices can be downloaded from the UF website:

\url{www.cise.ufl.edu/research/sparse/matrices/}

For the sparse triangular system examples, a matrix from the UF repository is first factorized and the resulting factor $L$ is stored in a local repository to be used in the triangular solve experiments. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}
The steps to installing Sympiler and then the setup instructions for Eigen and CHOLMOD are presented here.

\textit{\textbf{ Sympiler.}} Since the current version of Sympiler calls some BLAS routines, the user needs to modify the \textit{BLAS\_LIB} variable in \textit{CMakeLists.txt} and set it to the installed OpenBLAS library path. The following shows the remaining steps for installing Sympiler.
\begin{lstlisting}
$ git clone <will be provided upon acceptance> Sympiler  
$ cd Sympiler; 
$ mkdir build; cd build;
$ cmake ..
$ make
\end{lstlisting}

\textit{\textbf{ Libraries.}}  We have prepared a simple project for evaluating Cholesky and the triangular solver using Eigen and CHOLMOD libraries. After installing CHOLMOD and Eigen, the paths have to be set via \textit{CHOL\_LIB} and \textit{Eigen\_LIB} in \textit{libTest/CMakeLists.txt}. The following steps will prepare the test environment for evaluation. 
\begin{lstlisting}
$ cd libTest; 
$ mkdir build; cd build;
$ cmake ..
$ make
\end{lstlisting}

As indicated in the paper, node amalgamation is disabled in CHOLMOD for fair comparison. The final matrix format conversion from blocked to column compressed, which is by default a part of the CHOLMOD numerical manipulation time, is also disabled. Thus, the reported time is only for the numerical manipulation of the actual factorization operation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}

\textit{\textbf{ Sympiler.}} We have prepared a script which generates the performance results for each algorithm evaluated in the paper. For the triangular solver, the user can run:
\begin{lstlisting}
$ cd /path/to/Sympiler/build/
$ ./triangular.sh  /path/to/triangular/input/matrix.mtx
\end{lstlisting}

The $triangular$ script first generates a code for the given matrix and stores it in the $symGen$ folder. Then it compiles and runs the generated code for the input matrix. For the Cholesky factorization, the user can run a separate script as follows:

\begin{lstlisting}
$ ./cholesky.sh  /path/to/input/matrix.mtx
\end{lstlisting}

\textit{\textbf{ Libraries.}} To compare Sympiler's performance with the two libraries, two binary files one for each algorithm in \textit{libTest} are provided. These files are built from the source code available in the repository. For triangular solve evaluation, the following sequence of commands will show the execution time of Eigen and Sympiler. Functions are provided within the code that verify the correctness of the resulting vector \textit{x}.
\begin{lstlisting}
$ cd /path/to/Sympiler/libTest/build/
$ ./libTriangular  /path/to/triangular/input/matrix.mtx
\end{lstlisting}
For the Cholesky evaluations, the following commands show the performance of both Eigen and CholMod libraries for a given input matrix. A built-in function compares the \textit{L} factor to check correctness. 
\begin{lstlisting}
$ cd /path/to/Sympiler/libTest/build/
$ ./libCholesky  /path/to/input/matrix.mtx
\end{lstlisting}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

The expected results include the factor $L$ for Cholesky and the solution vector $x$ for the triangular solver. The performance results include the numerical manipulation and the symbolic analysis time which are also presented in FLOPS. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment customization}

The experiments can be easily ran for other \textit{matrix market} matrices. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notes}
An updated installation guide will be provided in the Sympiler repository. 

==> artifactCodeStyle.tex <==
\lstset{ %
language=Bash,                % choose the language of the code
basicstyle=\ttfamily\footnotesize,       % the size of the fonts that are used for the code
columns=fullflexible,
numbers=left,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=0,                   % the step between two line-numbers. If it is 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
%backgroundcolor=\color{codeBG3},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,           % adds a frame around the code
tabsize=2,          % sets default tabsize to 2 spaces
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=false,    % sets if automatic breaks should only happen at whitespace
escapeinside={\%*}{*)},          % if you want to add a comment within your code
keywordstyle=\bfseries,       % keyword style
  %language=Octave,                 % the language of the code
  otherkeywords={git,mkdir,make,cmake,...},           % if you want to add more keywords to the set
  numberstyle=\tiny\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},
  escapechar=|
}


